Planar rooted line arrangements and an operad for factorized scattering

We introduce two topological non-$\Sigma$ operad structures on planar line arrangements subject to a certain geometric order condition, ensuring a well-defined notion of particle ordering on a distinguished line. This is interpreted in terms of scattering diagrams in purely elastic (1+1)-dimensional theories. We discuss a possible approach to factorized scattering in operadic terms.

==> blue_cor.tex <==
\begin{tikzpicture}[scale=1, grow=up, level distance=1cm, sibling distance=1.5cm, inner sep=2mm]

\node[draw=none] {}
child 
{
node[circle, draw, fill=cyan!40] (B1) {}
child { node (B4) {\Large 2} }
child { node (B5) {\Large 1} }};

\end{tikzpicture}

==> parallel.tex <==
\begin{tikzpicture}[inner sep=2mm]

\node[draw,circle] (A) at (0,0) {$+$};
\node[draw,circle] (B) at (2,0) {$-$};    

% Edges
\draw[->, bend left=50] (A) to node[above] {1} (B);  
\draw[->, bend right=50] (A) to node[below] {2} (B);

\end{tikzpicture}




==> red_cor.tex <==
\begin{tikzpicture}[scale=1, grow=up, level distance=1cm, sibling distance=1.5cm, inner sep=2mm]

\node[draw=none] {}
child 
{
node[circle, draw, fill=red!40] (B1) {}
child { node (B4) {\Large 2} }
child { node (B5) {\Large 1} }};

\end{tikzpicture}

==> series.tex <==
\begin{tikzpicture}[scale=1, grow=up, level distance=1.2cm, sibling distance=2cm, inner sep=2mm,
level 3/.style={sibling distance=0.6cm}]
    \node[draw,circle] (A) at (0,0) {$+$};
    \node[draw,circle] (B1) at (1,0) {};    
    \node[draw,circle] (C) at (2,0) {$-$};
    
    % Edges
    \draw[->] (A) to node[below] {1} (B1);
    \draw[->] (B1) to node[below] {2} (C);
   
\end{tikzpicture}
